Context-Adaptive Hearing Aid Fitting Advisor through Multi-turn Multimodal LLM Conversation

Traditional hearing aids often rely on static fittings that fail to adapt to their dynamic acoustic environments. We propose CAFA, a Context-Adaptive Fitting Advisor that provides personalized, real-time hearing aid adjustments through a multi-agent Large Language Model (LLM) workflow. CAFA combines live ambient audio, audiograms, and user feedback in a multi-turn conversational system. Ambient sound is classified into conversation, noise, or quiet with 91.2\% accuracy using a lightweight neural network based on YAMNet embeddings. This system utilizes a modular LLM workflow, comprising context acquisition, subproblem classification, strategy provision, and ethical regulation, and is overseen by an LLM Judge. The workflow translates context and feedback into precise, safe tuning commands. Evaluation confirms that real-time sound classification enhances conversational efficiency. CAFA exemplifies how agentic, multimodal AI can enable intelligent, user-centric assistive technologies.

==> data/tables/knowledge-fields.tex <==
\begin{table}
  \caption{Description of attributes to be filled by Strategy Provider agent.}
  \label{tab:knowledge_fields}
  \begin{tabular}{l p{4.8cm}}
    \toprule
    \textbf{Attribute} & \textbf{Description/Options} \\
    \midrule
    Adaptation Period & \{'External', 'Internal'\} \\
    Contraindications & \{'Recurrence', 'No Recurrence'\} \\
    Sound Source & \{'Television/Electronic Device/Other'\} \\
    Positive Benefit & \{'No Problem', 'Problematic'\} \\
    Volume & \{'Sufficient', 'Insufficient'\} \\
    Low-Frequency Impact & \{'Muffled', 'Not Muffled'\} \\
    Audiogram Shape & \{'Steeply Slope', 'Flat', 'Gently Slope', 'Rising'\} \\
    Gender Voice & \{'Male/Female', 'Clear/Unclear'\} \\
    \bottomrule
  \end{tabular}
\end{table}

